Storm: a fast transactional dataplane for remote data structures

RDMA is an exciting technology that enables a host to access the memory of a remote host without involving the remote CPU. Prior work shows how to use RDMA to improve the performance of distributed in-memory storage systems. However, RDMA is widely believed to have scalability issues, due to the amount of active protocol state that needs to be cached in the limited NIC cache. These concerns led to several software-based proposals to enhance scalability by trading off performance. In this work, we revisit these trade-offs in light of newer RDMA hardware and propose new guidelines for scaling RDMA. We show that using one-sided remote memory primitives leads to higher performance compared to send/receive and kernel-based systems in rack-scale environments. Based on these insights, we design and implement Storm, a transactional dataplane using one-sided read and write-based RPC primitives. We show that Storm outperforms eRPC, FaRM, and LITE by 3.3x, 3.6x, and 17.1x, respectively, on an Infinband EDR cluster with Mellanox ConnectX-4 NICs.

==> breakdown.tex <==
\label{section:EndToEndBreakdown}
%Remote Direct Memory Access (RDMA)~\cite{todo} is used in existing systems
%to enable fast and efficient communication among servers in a datacenter.
%We briefly explain the usage of Network Interface Controller
%(NIC) from Melanox~\cite{todo}, which utilizes RDMA-support of modern CPUs.
Servers with RDMA support communication with each other using \emph{queue
pairs (QPs)}, where each queue pair consists of two \emph{work queues
(WQs)}: a \emph{send} and a \emph{receive} queue. The QPs are created by
applications, using the \emph{verbs} API, which applications can also use to
issue verbs (i.e., operations) to the one of the WQs. Issuing a verb
consists of creating a \emph{work queue element (WQE)} and inserting the
WQE to the QP.  The RDMA controller processes WQEs in a QP by generating a network request for each of them. The remote RDMA controller, on the other hand, receives the requests, processes them, and notifies the sender RDMA controller about the completion of the request. Upon receiving the notification message, the sender RDMA controller creates a \emph{completion queue entry (CQE)} and inserts it into the \emph{completion queue (CQ)}. RDMA can be used to implement both storage-level and memory-level SM.

A NIC typically communicates with the CPU chip over a PCIe bus.
Figure~\ref{fig:rdma_nic} shows a system with RDMA NIC and steps of data
replication using the NIC. To write data to the memory of the replica
server, the CPU first needs to create a WQE~\circled{1} and then insert it to the SQ~\circled{2} ($T_{CPU\_insert\_WQE}$). The WQE
contains the type of the request (i.e., a memory write in this case) and
the data inlined in the WQE or a pointer to the data instead. Once the WQE
is inserted into the SQ, the NIC driver sends the WQE to the NIC over the
PCIe bus. The driver may send the WQE directly using \emph{Memory Mapped IO
(MMIO)}, which we do not show in the figure, or it may just send a short
message using MMIO to tell the NIC
where to read the WQE from, referred to as \emph{doorbell ring}~\circled{3} ($T_{CPU\_ring\_doorbell}$). 
The former approach is more efficient for small message sizes as the content of the WQE is inlined and there's only one PCIe traversal. The latter approach is more efficient for larger message sizes, as the 
PCI header overhead is amortized across multiple WQEs. In our analysis, we focus on the latter approach as we expect to perform SM updates at coarse granularities. %Note that
%sending the WQE directly with a large MMIO message may keep the CPU busy for
%significant amount of time. 
%In contrast, because the doorbell message is
%relatively small, sending a doorbell message would consume less CPU time.


When the local NIC receives a doorbell ring, the NIC initiates a DMA operation to
read one or more WQEs from the cache~\circled{4} ($T_{lNIC\_read\_WQE}$). Upon receiving the WQE, the NIC
processes it~\circled{5} . If the data is inlined within the WQE, the NIC can directly
issue a request into the network for a write to the remote NIC.
Otherwise, the local NIC needs to initiate a second DMA operation~\circled{6} to
read the data from the memory using the pointer obtained from the WQE.
Since RDMA works with virtual addresses, address translation is a necessary step 
whenever the NIC requires access to memory. The NIC is equipped with a Memory Management Unit (IO-MMU) featuring 
its own translation buffer. 
Aside from the translation buffer, the NIC also features an SRAM cache for Memory Translation Table (MTT) and QP entries.
%to cache address translation entries.
Due to the limited amount of SRAM cache available on the NIC, the NIC often requires additional
memory accesses to fetch the MTT or QP entries
%and perform address translation upon 
%a IO-TLB miss. 
Such additional PCIe transmissions introduce variable latency and increase the overall latency of RDMA operations. We represent this overall latency as $T_{lNIC\_proc\_WQE}$.

After fetching the data ($T_{DMA\_read\_data}$), the NIC issues a request to the
network~\circled{7} ($T_{IB\_trans\_data}$), which is
received and processed by the NIC of the replica server ($T_{rNIC\_proc\_request}$). In the replica
server, the NIC sends the data to the DMA over the PCIe bus, and the DMA
writes the data to the target memory address~\circled{8} ($T_{DMA\_write\_data}$). After posting a PCI write, the
remote NIC issues a completion message to the network~\circled{9} ($T_{IB\_trans\_ACK}$).
That message propagates back
to the local NIC, which processes it ($T_{lNIC\_proc\_ACK}$) and creates a CQE~\circled{10}, and
finally inserts it into the CQ~\circled{11} ($T_{lNIC\_insert\_CQE}$). The remote RDMA write operation ends with the CPU processing the CQE ($T_{CPU\_proc\_CQE}$).
Equation~\ref{eqRDMA} provides the latency model of a simple RDMA write operation:

%\todo{Is this correct? I thought that the remote RNIC does not wait for the memory write to complete. I see that you address this later, should we foreshadow that here?}

%The PCIe Max Payload Size determines the maximal size of a PCIe packet, or PCIe MTU (similar to networking protocols). This means that larger PCIe transactions are broken into PCIe MTU sized packets. This parameter is set only by the system and depends on the chipset architecture (e.g. x86_64, Power8, ARM, etc). You can view the PCIe Max Payload Size by using the command lspci (specified under DevCtl).


%In this section we assuem a simple analyze the latency components of a simple replication scenario with different message sizes. 



\begin{equation}
\label{eqRDMA}
\begin{split}
T_{RDMA} &= T_{CPU\_insert\_WQE}  + T_{CPU\_ring\_doorbell} \\
                    & +  T_{lNIC\_read\_WQE} + T_{lNIC\_proc\_WQE} + T_{DMA\_read\_data}\\
                    & + T_{IB\_trans\_data} + T_{rNIC\_proc\_request} +T_{DMA\_write\_data}\\
                    & + T_{IB\_trans\_ACK} + T_{lNIC\_proc\_ACK} + T_{lNIC\_insert\_CQE}\\
                    & + T_{CPU\_proc\_CQE}
\end{split}
\end{equation}

% Then we analyse the latency results of a simple mirroring scenario and provide latency breakdown to indentify of the contribution of different mirroring steps.

In the above latency equation~\ref{eqRDMA}, some components are constant and some vary depending on the message size, access pattern, and network bandwidth.
Accordingly, we can rewrite Equation~\ref{eqRDMA}
as Equation~\ref{eqRDMA2} where $T_{constant}$ includes the time required to accomplish the constant latency steps.

\begin{subequations}
\label{eqRDMA2}
\begin{equation}
\label{eqRDMA2a}
\begin{split}
T_{RDMA} &= T_{constant}\\
                 & + T_{lNIC\_proc\_WQE}+T_{DMA\_read\_data} \\
                 & + T_{IB\_trans\_data}+T_{rNIC\_proc\_request}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
T_{costant} &= T_{CPU\_insert\_WQE} + T_{ring\_doorbell} \\         
                & +T_{lNIC\_read\_WQE} + T_{IB\_trans\_ACK} \\
                & + T_{lNIC\_proc\_ACK} + T_{lNIC\_insert\_CQE} \\ 
                & + T_{CPU\_proc\_CQE}
\end{split}
\end{equation}
\end{subequations} 

However, when the message size is larger than the IB MTU (on our evaluation platforms 4KB for Platform-1 and 1500 bytes for Platform-2) different steps of RDMA transfer can be executed in parallel. In fact, when the size of the read data is equal to MTU, then the NIC can start data transmission while the remaining data chunks are being DMA'ed. The slower of the two operations (RDMA transfers and the DMA reads) ends up determining the overall latency.
We represent the time taken to DMA read and RDMA transfer an MTU sized message as $T_{DMA\_read\_MTU}$ and $T_{IB\_trans\_MTU}$ respectively.
In addition, we learn that under the Reliable Communication mode in Infiniband, which is mandatory for remote reads and writes to work, the remote NIC does not wait for the DMA write (\circled{8} in Figure~\ref{fig:rdma_nic}) to complete and hence can be omitted from the latency equation. Based on these observations, for a given message size $S$, network link bandwidth of $BW\_IB$, and PCIe bus bandwidth of $BW\_PCIe$, we can rewrite Equation~\ref{eqRDMA2} as Equation~\ref{eqRDMALarge}:
%So, we can just replace the the latency Equation~\ref{eqRDMA2} can be rewritten as:
%\begin{equation}
%\label{eqRDMA2a}
%\begin{split}
%T_{RDMA} &= T_{constant}\\
                 %&+ %T_{DMA\_read\_data}+T_{IB\_trans\_data}+T_{DMA\_write\_%data}
%\end{split}
%\end{equation}
%As depicted in Figure~\ref{todo},


%\begin{equation}
%\label{eqRDMALarge}
%\begin{split}
%T_{RDMA} &= T_{constant}\\
%                     & + \frac{S}{MTU}\times T_{DMA\_read\_MTU} \\
%                     & + T_{IB\_MTU\_packet} + T_{DMA\_write\_MTU}
%\end{split}
%\end{equation}



\begin{equation}
\label{eqRDMALarge}
\begin{split}
T_{RDMA} =& T_{constant} + T_{lNIC\_proc\_WQE} +T_{rNIC\_proc\_request}\\
          & + T_{DMA\_read\_MTU} \\
          & + T_{IB\_trans\_MTU} + ceil\left(\frac{S - MTU}{\min(BW\_{IB}, BW\_{PCIe})}\right)
\end{split}
\end{equation}

For the ceiling of the fraction in Eq~\ref{eqRDMALarge}, we use a min value of zero. 

For SM to guarantee correctness, the data written to remote memory must be persistent. However, since the RNIC does not wait for remote writes to complete and replies to the 
sender ahead of time, RDMA does not provide SM persistency guarantees and requires special support, similar to $clwb$, but a remote version of it. In addition to correctness issues, 
RDMA generally suffers from a high-overhead hardware-software interface -- PCIe bus, which 
can slow down SM. RDMA write operations require multiple PCIe transmissions for control 
and data access purposes. Through this work we identified address translation as a key source of additional PCIe overhead. Finally, the variable parameters in the above equations
can vary significantly depending on whether there is interference with other applications
collocated on the same server. Current RNIC implementations do not provide sufficient
isolation at the level of WQE scheduling, which affects the performance of SM.

The analysis presented above can be used to model the scenario of one outstanding RDMA write request in an unloaded network. While such a model may be too simplistic to model a generic RDMA network flow, it is representative of the network traffic 
that we observed while employing memory-level SM for WHISPER applications. These applications have very few outstanding requests (due to frequent syncrhonization points) and due to the small fraction of writes to persistent memory (less than 5\%) generate few RDMA writes leading to an uncongested network. 
We build our performance model based on this observation, validate it with measurements from our platform and then use it to figure out the architectural bottlenecks. We describe our model next.

%\todo{\textbf{Discussion- RDMA deficiencies:} Why is RDMA as currently constitutes not good enough? What needs to be changed? What are the implications of those changes on the above equations?}

%In the following section, we describe the design and implementation of our cycle-accurate model of an RDMA network and validate it using our RDMA platforms.

%\begin{equation}
%\label{eqRDMALarge}
%\begin{split}
%T_{RDMA} &= T_{constant}\\
%                    & + \frac{S}{MTU}\times T_{DMA\_read\_MTU} + T_{IB\_MTU\_packet} + T_{DMA\_write\_MTU}
%                    &+ \frac{S}{max\_read\_size}\times T_{max\_read\_req}+\frac{S}{max\_payload}\times T_{max\_read\_comp}\\
 %                &+\frac{S}{MTU}\times T_{IB\_packet}+\frac{S}{max\_payload}\times T_{write\_req}\\
%                &= T_{constant}\\
 %               &+S\times\Big(\frac{T_{read\_req}}{max\_read\_size}+\frac{ T_{IB\_packet}}{MTU}+\frac{T_{read\_comp}+T_{write\_req}}{max\_payload}\Big)
%\end{split}
%\end{equation}









==> interference.tex <==
\label{section:PerformancePredictabilityStudies}

\begin{table*}[h!]
\caption{Summary of the microbenchmarks used to analyze the interference between memory-level SM applications.} 
%\caption{Our RDMA platforms}
\centering 
\renewcommand{\arraystretch}{1.4} 

\begin{tabular}{|m{4cm} m{2.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm}|}
\hline
\textbf{Microbenchmark} & \textbf{Access pattern} & \textbf{No. of Processes} &
\textbf{Request size} & \textbf{Batch size} &
\textbf{Working set size} &
\textbf{Designed to test}\\
\hline 
1P-1GB-Random & Random & 1 & 64B & 1 & 1GB & MTT \\
1P-1GB-Streaming & Streaming & 1 & 64B & 1 & 1GB & MTT\\
\hline
16P-64MB-Random & Random & 16 & 64B & 1 & 64MB each & QPs \\
16P-64MB-Streaming & Streaming & 16 & 64B & 1 & 64MB each & QPs\\
\hline
1P-64MB-Constant & Constant & 1 & 16KB & 32 & 64MB & PCIe\\
\hline
\end{tabular}
\label{table:microbenchmarks}

\end{table*}

In this section, we consider the interference that could occur between applications that are using the same RNIC for memory-level SM. 
To understand the sources of this interference better, we run the WHISPER applications in conjunction with a variety of microbenchmarks.
The microbenchmarks are:

\textbf{1P-1GB-Random:} One process making random remote accesses to a 1GB buffer with a batch size of one. We designed this microbenchmark to test the contention between the applications at the MTT.

\textbf{1P-1GB-Streaming:} One process making streaming remote accesses on a 1GB working set with a batch size of one. We designed this microbenchmark to test the contention between the applications at the MTT. 

\textbf{1P-64MB-Constant:} One process making constant accesses on a 64MB working set with a batch size of 256 cache blocks. We designed this microbenchmark to test the contention between the applications at the PCIe bus.

\textbf{16P-64MB-Random:} Sixteen processes making random accesses on their private 64MB working set with a batch size of one. The working sets are non-overlapping and cumulatively add up to 1GB. We designed this microbenchmark to test the contention between the applications at the Queue Pairs (QPs).

\textbf{16P-64MB-Streaming:} Sixteen processes making streaming accesses on their private 64MB working set with a batch size of one.The working sets are non-overlapping and cumulatively add up to 1GB.We designed this microbenchmark to test the contention between the applications at the QPs.

We summarize the properties of these microbenchmarks in Table~\ref{table:microbenchmarks}. Running various WHISPER applications in conjunction with our microbenchmarks lead us to the following observations.


\begin{figure}[!t]
  \centering
\quad\includegraphics[angle=0,width=0.80\columnwidth]{figures/5-QoS-MTT-Key.pdf}\vspace{-3mm}
\subfloat[\texttt{Platform 1}]{\label{fig:QoS:MTT:IB}{
            \includegraphics[angle=0,width=0.85\columnwidth]{figures/5-QoS-MTT-IB-ExecutionTime.png}}}\vspace{-3mm}\\
\subfloat[\texttt{Platform 2}]{\label{fig:QoS:MTT:RoCE}{
            \includegraphics[angle=0,width=0.85\columnwidth]{figures/5-QoS-MTT-RoCE-ExecutionTime.png}}}\vspace{-2mm}
  \caption{The normalized execution times of various WHISPER applications when run in conjunction with our microbenchmarks on both platforms. The execution times are normalized to the case where each application is running stand-alone.}
\label{fig:QoS:MTT}
\end{figure}

\textbf{Lightweight applications do not interfere with WHISPER applications:}
Of all our microbenchmarks, 1P-1GB-Streaming was designed to interfere least with the WHISPER applications. As can be seen from Figure~\ref{fig:QoS:MTT}, on both of our platforms, 1P-1GB-Streaming causes only modest increases (< 10\%) in execution times.
This behavior is to be expected, as 1P-GB-Streaming causes very little contention at the MTT or the QPs or the PCIe bus.

\textbf{WHISPER applications are insensitive to MTT thrashing:}
We designed 1P-1GB-Random to contend with concurrent applications at the MTT, but introduce very little contention at the PCIe bus or the QPs.
As can be seen from Figure~\ref{fig:QoS:MTT}, on both of our platforms 1P-1GB-Random introduces little performance degradation.
In fact, the execution times achieved by application when run together with 1P-1GB-Random is very similar to the the execution times seen with 1P-1GB-Streaming, a microbenchmark designed to not thrash the MTT. 
The performance similarity between random and streaming access patterns can also be seen with microbenchmarks with 16 processes (16P-64MB-Random and 16P-64MB-Streaming)
These observations lead us to believe that WHISPER applications, even with working set sizes larger than 1GB, are insensitive to MTT thrashing.
%(\todo{Shouldn't we be doing 1P-1GB-Constant also?})
%\todo{Stanko: by insensitive do you mean they already thrash the MTTs, and the micro-benchmarks do not add much?}

\textbf{The lack of support for QoS at the QP level negatively impacts the performance of WHISPER applications:}
We designed the microbenchmarks with 16 processes (16P-64MB-Random and 16P-64MB-Streaming) to analyze how the scheduling of WQEs inside the RNIC affects overall performance.
As can be seen from Figure~\ref{fig:QoS:MTT}, on average, the 16 process microbenchmarks cause higher performance degradation (about 50\% on Platform-1 and 40\% on Platform-2) than the 1 process microbenchmarks.
The 16 process microbenchmarks issue many concurrent RDMA requests leading to contention for the available WQEs.
RNIC's with better support for QoS can isolate different applications from the interference caused by the other applications.
In fact, we believe that the better performance of applications when run together with the 16 process microbenchmarks on Platform-2 (Figure~\ref{fig:QoS:MTT:RoCE}) than on Platform-1 (Figure~\ref{fig:QoS:MTT:IB}), 40\% slowdown vs 50\% slowdown, is due to better support for QoS in the ConnectX-4 RNIC on Platform-2 than ConnectX-3 RNIC on Platform-1. We confirm our hypothesis through personal communication with Mellanox~\cite{personal}.

%\todo{Shouldn't we run experiments with different no. of processes so that we can show where this support for QoS starts mattering?}


\textbf{Network contention throttles performance:}
We designed 1P-64MB-Constant to assess the impact of network contention on the performance 
of WHISPER applications.
1P-64MB-Constant, accesses the same addresses over and over again, perfectly utilizing the MTT and sparingly using the QPs. 1P-64MB-Constant benchmark issues 32 RDMA write requests at a time, where each request is 256 cache blocks in size, consuming almost all available bandwidth and making the network the major source of contention.
Figire~\ref{fig:qos_pcie} illustrates the severe performance degradation of WHISPER applications on both of our platforms 2.2x on Platform-1 and 2.4x on Platform-2 on average) when run alongside 1P-64MB-Constant.
%due to the lack of support for QoS at the network level. 1P-64MB-Constant benchmark is designed to consume all the bandwidth, thus leading to network saturation.
A well-designed network is supposed to provide QoS guarantees across all running applications and share the available network bandwidth in a fair manner. With current RNIC implementations, a process aggressively using the network can easily preempt other applications and degrade their performance, as illustrated on Figure~\ref{fig:qos_pcie}.

Next, we take a deeper dive into the architectural and RDMA design choices that lead to the sub-optimal performance of memory-level SM.

%(\todo{xx} in total)
%is the PCIe bus as 1P-64MB-Constant transfers large messages (\todo{xx} bytes) over the PCIe bus to the RNIC.
%\todo{Completion pending results.}


\begin{figure}[] \centering
\includegraphics[angle=90,width=0.98\linewidth]{figures/5-QoS-PCIe.pdf}%
%\vspace{-.05in}
\caption{Performance impact on WHISPER applications when the network bandwidth becomes a bottleneck.}
\label{fig:qos_pcie}
%\vspace{-.1in}
\end{figure}


%\todo{Again, shouldn't we doing a sweep of message sizes?}


==> new_design.tex <==
\label{section:newDesign}
We provide a brief overview of a new kind of the RNIC designed
for SM. In this paper, we learned that current RNIC implementations sacrifice QoS for the 
sake of direct, user-level hardware-software interface and leverage PCIe/DMA to directly access local memory. We find that such design severely
impacts the performance of SM, and, thus, we argue for an integrated version of the
RNIC that minimizes the overhead of QP interactions and address translation. 
We believe that the imporved RNIC design should use a special DMA interface and a protocol to reduce the number of messages exchanged between the memory hierarchy and the network interface compared to what is incurred with PCIe.  


\textbf{RNIC design for memory-level SM:}
We propose an integrated version of the RNIC that consists of two dependent 
architectural components: (i) the RNIC front-end (RNIC-FE) consists of the control logic 
that implementes WQE processing, completions, and address translation; (ii) RNIC
back-end (RNIC-BE) that is essentially an Ethernet NIC or the equivalent, special version of the L3-only Infiniband HCA. The hardware-software interface is identical to RDMA, as the
RNIC-FE implements the IB transport protocol. 
The RNIC-FE is tightly integrated with the processor and is located on-chip, making sure that the PCIe does not get in the way of address translation, QP interactions, and 
data reads/writes. The RNIC-BE is connected with the RNIC-FE via a low-latency, high-bandwidth bus that DMAs IB packets directly from the CPU cache and injects them into the network.
%We do not disclose the details of the bus, nor the microarchitecture as this
%is work-in-progress.
The benefit of such split design is two-fold: (i) there is a minimial number of messages exchanged over the bus because of the on-chip RNIC-FE and, hence, there is no trashing (all metadata, including MTT and QP is in the CPU cache), and (ii) the transfer is not bound by the latency of the PCI bus, which we identified as the key source of overhead in SM.

To estimate the performance impact of these RNIC improvements require a deep micro-architectural analysis that is beyond the scope of this paper and require a cycle-accurate architectural simulator.
The design and the performance modeling of this new RNIC design is currently work-in-progress.


%\noindent\textbf{Microarchitectural SM RNIC simulator.}
%\todo{
%Gem5 is frequently used by computer architects to model various hardware innovations and estimate their affect on performance, energy, etc.
%We extend standard gem5 with a RNIC hardware module and connect it to the PCIe bus interface. We also develop an RDMA driver to help applications running on gem5 to communicate with our RNIC module.
%We simulate a remote machine with the same RNIC hardware and develop the network module to allow communication between the two RNICs.
%}

% From Many-core NI, ISCA 2015: Unlike traditional implementations of RDMA, which operate over the PCI bus, the RMC benefits from a tight integration into the processor’s cache coherence hierarchy. In particular, the processor and the RMC share all data structures via the cache hierarchy. The implementation of the RMC is further simplified by limiting the architectural support to one-sided remote memory read, write, and atomic operations, and by unrolling multi-line requests at the source RMC. As a result, the protocol can be implemented in a stateless manner by the destination node

%Unlike a traditional RDMA NIC, the RMC has direct access to the page tables managed by the operating system, leveraging the ability to share cache-coherent data structures. As a result, the RMC and the application both operate using virtual addresses of the application’s process once the data structures have been initialized


==> old_intro.tex <==


% importance of durability and availability
Durability and availability are among the most critical properties of the modern cloud and datacenter services, since a loss of data or even a very short service outage can lead to serious financial consequences and also cause consumer dissatisfaction~\cite{bilal2014trends,Book:ManagingMicrosoftHybridCloud}. Common issues that have negative effect on durability and availability are outages that may arise due to external factors (e.g., interruption in power supply or network downtime) or faults that are common in hundreds to thousands of processing, networking, and storage components of the modern datacenter infrastructures. A fault can lead to data-loss or unavailability in different levels (e.g., server, rack, datacenter), and thus ensuring datacenter-wide high fault-tolerance is critical to guarantee highly-durable and highly-available datacenter services. 

% Data mirroring as a technique to provide high durability/availability
% Mirroring at different hardware unit levels (servers, racks, datacenters)
A technique that datacenters commonly implement to provide high-durability and high-availability is maintaining multiple 
copies of the user application \emph{persistent}  state. This technique of replicating data of the \emph{main} server (that runs user application) into multiple \emph{replica} servers is called \emph{data mirroring}. Typically, the
durability and availability that mirroring can provide improve with the
increase of physical distance between the main and replica servers, since the servers at close proximity share resources that in case
of a failure affect all servers sharing it.  Specifically, servers
inside a rack share the same power supply and top-of-rack (ToR) network 
switch~\cite{Book:ManagingMicrosoftHybridCloud}, which makes them belonging to the same \emph{fault
domain}. Mirroring inside a rack can protect against single-server
failures but, in case of a fault in the power supply or ToR, the entire rack would be
unavailable. Thus only a replica in a different fault domain (i.e., rack) can prevent
data loss and keep the services available. Similarly, a datacenter may also
be considered as a high-level fault domain, and mirroring can be performed
between servers from different datacenters. 


% Shall we tell about the performance (latency) overhead of mirroring?
% Expecially, the fact that latency increases when mirroring is applied at
% higher hardware unit level (intra-rack mirroring has lower performance
% overhead compared to inter-rack mirroring).

%However, latency of the mirroring becomes higher with the increase in the
%distance between the servers used for data mirroring due to the increasing
%communication cost, which may critically degrade the performance of
%datacenter services.  Thus, the mirroring should incur minimal performance
%overhead to the running services in a datacenter.


% Types of data mirroring (synchronous vs asynchronous)
Data mirroring mechanisms are generally categorized as \emph{synchronous}
and \emph{asynchronous} mirroring. In synchronous mirroring, a write
request is only committed after the data is written to the persistent
storages of both main and replica servers. Such a model ensures that the
main and replica copies are always identical, thus the most-recent version of the data
can always be fetched from replica server in case of main server failure. However, synchronous
mirroring provides such strong consistency at the expense of additional
write latency in the main server, which is incurred due to the round-trip latency of sending write data to the replica server and receving back the acknowledgement of the replica write.  In contrast, asynchronous mirroring allows temporary divergence between the main and replica storages by commiting a write request right after the data is written to the storage of \emph{only} the main server (not waiting for the replica write to be accomplished). Although asynchronous mirroring typically offers better write performance compared to synchronous mirroring, the weak-consistency model that asynchoronus mirroring provides does not always match the requirements of a datacenter application. Many business-critical and high-end transactional applications can not even tolerate the loss of a single write operation and as a result require a strong consistency between the main and replica copies of their state~\cite{Unterbrunner:2014:HAE,Dynamo-SOSP-2007}. A strongly-consistent
mirroring is also required for seamless failover from the main to replica
server, and for transparent live migration of virtual machines (VMs) in
highly virtualized datacenters~\cite{VMware-FT-2016}. 

Existing datacenters typically provide storage-level persistence where application data is stored on hard disk drives (HDD)s and solid-state drives (SSD)s, which have write latency in the range of \SI{500}{\micro\second} - \SI{10}{\milli\second}~\cite{Mellanox-NVMf-2016,Microsoft-RDMA-Extensions-2016}. Storage-level synchronous mirroring incurs latency overhead due to 1) the need to communicate data over the network, 2) the additional processing, which is required by software protocols that enable mirroring, at the main and replica servers, 3) the write operations performed at the storage devices of the replica servers, and 4) the need to send write acknowledgment from the replica server back to the main server.
However, the latency overhead of the replication is insignificant since the latency of the network communication and mirroring protocols is relatively small compared to the write latency of the storage  devices (5-20\%)~\cite{Mellanox-NVMf-2016,Microsoft-RDMA-Extensions-2016}. 


\juan{Part of the next paragraphs could be used for a short background on NVM}
Emerging non-volatile memory (NVM) technologies, such as Phase
Change Memory (PCM)~\cite{todo}, Spin-Transfer Torque RAM
(STT-RAM)~\cite{todo}, and Resistive RAM (RRAM) have introduced new level of persistent storage. They offer disk-like persistence with DRAM-like access latency and interface (i.e., byte-addressable access via load and store
instructions), low idle power, and better scalability compared to
DRAM~\cite{PMM-CACM-2010,PMM-IMW-2013-2}. Many proposals and prototypes for future systems
already employ low-latency NVM as a part, if not solely, of the main memory~\cite{SNIA-White-Paper-2016,PMM-2013,PMM-ICCD-2014,PMM-ISCA-2009,PMM-ISCA-2009-2,PMM-ISCA-2009-3,PMM-Micro-2010,PMM-ISPASS-2013}, which is traditionally implemented using
Dynamic Random Access Memory (DRAM). Consequently, Non-Volatile Main Memory (NVMM) enables \emph{memory-level persistence}.  Projections have shown that the latency of NVMM may approach that of DRAM~\cite{PMM-Micro-2010,PMM-ISPASS-2013,PMM-CACM-2010,PMM-IIEDM-2005,PMM-Patent-2004} and thus the latency of memory-level persistent storage would be two to three orders of magnitude faster than traditional storage devices. Previous work showed 10-100x performance improvement when slow HDDs are replaced with NVM, e.g. PCM, for persistent data storage~\cite{PMM-2013}. Synchronous mirroring of the memory-level persistent data would be a great challenge since the aggregate overhead of the replication protocol stack and network communication will be one to two orders of magnitude higher than that of the NVMM store operation. 

Many recent studies tried to implement NVMM replication using modern Remote Direct Memory Access (RDMA) in order to eliminate the large overhead of the conventional mirroring mechanisms~\cite{RDMA-PMEM-SDC-2015,RDMA-PM-Requirements-HP-SDC-2014,Mojim-2015}. RDMA is one of the fastest and lowest-overhead mechanisms that provides the user application with an interface for accessing the main memory of a remote server. RDMA bypasses the Operating System (OS) and thus remote memory read/write requests are directly sent from user application to the RDMA-enabled Network Interface Card (RNIC). The whole communication protocol is offloaded into the RNIC so that the additional overhead of the data copy in OS protocol stack is eliminated, leading to \emph{zero-copy} remote communication~\cite{Barthels-RacScale-2015}, and remote memory access is accomplished with very low CPU overhead. 

In this work, we investigate the efficiency of memory-level persistent state synchronous mirroring using modern RDMA. While a single store operation into NVMM is typically handled in 

% RDMA based mirrroing
% What is the goal of this paper
We find that the (widening) speed gap among DRAM cells
presents an opportunity to reduce DRAM access latency. If
we can understand and characterize the inherent variation
in cell latencies, we can use the resulting understanding to
reduce the access latency for those rows that contain faster
cells. The goal of this work is to (i) experimentally char-
acterize and understand the impact of latency variation in
the three fundamental DRAM operations for cell access (ac-
tivation, precharge, and restoration), and (ii) develop new
mechanisms that take advantage of this variation to improve
system performance.

To this end, we build an FPGA-based DRAM testing in-
frastructure and characterize 240 DRAM chips from three
major vendors. We analyze the variations in the latency
of the three fundamental DRAM operations by operating
DRAM at multiple reduced latencies. Faster cells do not
get affcted by the reduced timings, and can be accessed re-
liably without changing their stored value; however, slower
cells cannot be reliably read with reduced latencies for the
three operations, leading to bit 
ips. In this work, we de-
ne a timing error as a bit 
ip in a cell that occurs due to
a reduced-latency access, and characterize timing errors in-
curred by the three DRAM operations. Our experimental
characterization yields six new key observations.
First, we find that significant variation is present

% What are the contributions of this paper
%We hope that our extensive analysis leads to other new mechanisms to improve DRAM performance and reliability. To facilitate this, we will make our characterization results for all tested DRAM chips and the FLY-DRAM simulator publicly available [10]. 

%Based on these major conclusions from our comprehensive analysis and characterization of 240 DRAM chips from three major DRAM manufacturers, we propose and evaluate a new mechanism,


%It experimentally demonstrates and characterizes the significant variation in latency of three fundamental DRAM operations (activation, restoration, and precharge) across different cells within a DRAM chip.

% Motivation for Synchronous Mirroring
% Use cases supporting the need for synchronous mirroring
%Different applications have different consistency requirements that are
%quantified by \emph{Recovery Point Objective (RPO)}, which is a metric defined as
%the maximum time interval prior to a failure, during which the data could
%acceptably be lost due to divergence between the storages of the main and
%replica servers~\cite{todo}. Synchronous mirroring provides strong
%consistency, which is required to support zero RPO for business-critical
%and high-end transactional applications~\cite{}. 

% However, synchronous mirroring brings
% significant performance overhead even in case of emerging non-volatile
% memories, which reduce the cost of persistent write operations from
% microsecond-level to nanosecond-level. In this work, we show
% inefficiencies in synchronous data mirroring in systems that include
% non-volatile main memory, and propose new mechanisms to mitigate these
% inefficiendies.


==> rdma_modeling.tex <==
\label{section:ExperimentalMethodology}

%To understand the performance characteristics of memory-level SM
%over RDMA, we design and evaluate a model of a state-of-the-art RDMA network. We first study the end-to-end latency of RDMA, based on our knowledge of its architecture and the Infiniband transport protocol.

In this section, we first provide simple arithmetic describing the key contributors to the latency of RDMA writes.
However, such analysis does not reflect all the intricacies of the RNIC implementation and requires further inspection. In fact, users are frequently forced to reason about the RNIC as a black box. While the hardware-software interface to the RNIC is known and well-documented, the hardware implementation is confidential.
Our aim is to model an RDMA network in a cycle-accurate interconnection network simulator - BookSim~\cite{booksim} using readily available information and information obtained through personal communication with Mellanox~\cite{personal}.
We design and validate our model using measurements from both of out platforms which implement different RDMA protocols (Infiniband and RoCE). We later use the model to gain insights into the architectural bottlenecks in memory-level SM. 

% The evaluation platform, CPU, RDMA NIC etc.
% put a table to easily show the components of the evaluation platform
%To characterize the latency distribution of the steps of
%synchronous mirroring via RDMA, we use servers with configuration as we
%present in Table~\ref{table:system_config}. We perform our experiments with
%two server nodes, connected via high-throughput InfiniBand switch.
%Table~\ref{table:system_config} also shows the read and write latency of several NVM
%technologies, which we assume to be used as persistent memory in future
%systems.

\subsection{End-to-end Latency Breakdown}
%In this section we will describe that RDMA NICs work as black box devices.
In this section we provide a simple RDMA performance model that captures key steps in a remote write operation. We identify constant
and variable latency contributors and provide a first-order approximation of how they affect the end-to-end latency for variable message sizes. We, then, implement this model in BookSim and validate it using our RDMA platforms. We start with a detailed explanation of how a classical RNIC operates and its programming interface


\begin{figure*}[] \centering
\includegraphics[width=0.98\linewidth]{figures/6-sync_mirroring_rdma.pdf}%
%\vspace{-.05in}
\caption{Steps involved in synchronous mirroring on RDMA-based system.}
\label{fig:rdma_nic}
%\vspace{-.1in}
\end{figure*}





%\todo{The description of the evaluation platform:
%\begin{itemize}
%\item The InifiniBand platform at Systems Group
%\item The RoCE platform at VMware
%\item The basic scenario of RDMA transfers: MMIO? or DMA? We think %that it is better to briefly clarify that MMIO is not a choice for enterprise systems with heavy IOPS requirements. What are the limitations of MMIO? What is the message size and what is maximum number of available buffer slots?
%\item The programming model includes cache flush, or the cache is write-through. In the first case the programmer can use flush instruction when he/she wants to make sure that the data will be written in persistent memory (and mirrored).
%\item Message size. In principle we want to replicate at cache block size. However, this might be inefficient for RDMA. It is necessary to batch many cache blocks. This is possible if the cache blocks that are evicted during one RDMA replication operation are batched together and transferred in the next RDMA replication operation.
%\item The basic scenario of multi-thread execution to show inter-thread interference: how many threads are there in the experiments? what is the 
%\end{itemize}
%}

%\begin{scriptsize} 
%\begin{table}[h!] 
%\caption{System configuration}
%\centering 
%\renewcommand{\arraystretch}{1.4} 

%\begin{tabular}{m{1.5cm} m{6cm}}
%\hline 
%Processor & Intel Xeon E5-2630\\ 
%\hline 
%Memory & X GB DDR3 ECC DIMMs? \\ 
%\hline
%NVM & \begin{tabular}{c | c | c}
%		\emph{Technology} & \emph{Read Latency} & \emph{Write
%Latency} \\
%		\hline
%		PCM & \SIrange{48}{70}{\nano\second} &
%\SIrange{140}{450}{\nano\second} \\
%		\hline
%		STT-RAM & \SIrange{2}{3}{\nano\second} &
%\SIrange{11}{25}{\nano\second} \\
%		\hline
%		RRAM & \SIrange{2}{6}{\nano\second} &
%\SIrange{100}{200}{\nano\second} \\
%      \end{tabular} \\

%PCM (\SIrange{48}{70}{\nano\second} read latency,
%\SIrange{140}{450}{\nano\second} write latency),
%STT-RAM(\SIrange{2}{3}{\nano\second} read latency, \SIrange{11}{25}{\nano\second} write
%latency), RRAM (\SIrange{2}{6}{\nano\second} read latency,
%\SIrange{100}{200}{\nano\second} write latency) \\
%\hline 
%PCIe & Intel Haswell-E PCIe\\ 
%\hline 
%Network & Mellanox RDMA ConnectX-3 NIC, Mellanox InfiniBand Switch with FDR support\\
%\hline
%\end{tabular}
%\label{table:system_config}
%\end{table}
%\end{scriptsize}

% PCM latency value references:
% + A 20nm 1.8v 8gb pram with 40mb/s program bandwidth, ISSCC'12
% + Phase Change Memory, Wong et al., IEEE, 2010
% There is a survey, maybe we can just cite it:
% + Architecting phase change memory as a scalable dram alternative, Lee et
% al, ISCA'09

% STT RAM latency value references:
% + Technology Comparison for Large Last-Level Caches (L3Cs): Low-Leakage
% SRAM, Low Write-Energy STT-RAM, and Refresh-Optimized eDRAM, Chang et
% al., HPCA'13
% + A Novel Architecture of the 3D Stacked MRAM L2 Cache for CMPs, Sun et
% al., HPCA'09 

% Memriston latency value references:
% + Design Implications of Memristor-Based RRAM Cross-Point Structures, Xu
% et al, DATE'11

% Describe the evaluation software (experiments, measurements)


% Latency overhead of RDMA, give detailed explanation of the components
% that introduce latency overhead
%We model the overall latency of a replicated storage write with synchronous
%mirroring as follows:

%$L_{Replication} = 2*(L_{LRM} + L_{BN} + L_{RRM}) + L_{Disk}$

%$L_{Disk} \simeq \SI{500}{\micro\second} - \SI{10}{\milli\second}$

%$2*(L_{LRM} + L_{BN} + L_{RRM}) < \SI{10}{\micro\second}$

%\todo{Update the equation above to have notation similar to the notation of
%the previous paragraph}


% Summarize by telling that we need communication architecture to enable
% mirroring more efficiently 

%The existing RDMA-based communication can be efficiently used to
%implement synchronous mirroring on storage-level. However, it has
%significant latency impact on memory-level synchronous mirroring.

\input{breakdown.tex}

\begin{figure}[!t]
  \centering
\subfloat[\texttt{booksim} model]{\label{fig:simulation_pictorial}\includegraphics[angle=0,width=0.9\columnwidth]{figures/6-simulation-pictorial.jpg}}\vspace{-4mm}\\
\subfloat[\texttt{Validation}]{\label{fig:validation}\includegraphics[angle=0,width=0.98\columnwidth]{figures/6-validation.pdf}}\vspace{-2mm}
  \caption{Validation of our RDMA model in Booksim against the results obtained on our RDMA platforms.}
\label{fig:simulation}
\end{figure}

\subsection{Cycle-accurate Simulation Model}
To better analyze the affect of RDMA network internals on overall performance, we model RDMA network in a cycle-accurate interconnection network simulator, \emph{booksim}~\cite{booksim}.
booksim can be used to faithfully model various different network topologies, routing algorithms and custom hardware designs. 
As shown in Figure~\ref{fig:simulation_pictorial}, we model our platforms as three separate nodes: 1) \emph{main-server} (hosting the local procesor and the PCIe controller), 2) \emph{local-RNIC}, and 3) \emph{remote-RNIC}.
The communication between the local-processor and the local-RNIC is modeled after the PCIe protocol, while the communication between the local-RNIC and the remote-RNIC is modeled after the RDMA protocol.
In the model, we use measurements from our platforms to configure the constant timing parameters and tune the rest of the system to match the overall end to end latencies measured on our platforms.


\subsection{Model Validation and insights}
We predict the end to end latencies observed for different message sizes (from 1 to 256 cachelines) using our model and compare them to the latencies measured on both of our platforms. 
Figure~\ref{fig:simulation} compares the measured and modelled latencies on both of our platforms and also plots the error in our modeled latencies (as a fraction of overall latency).
Our model is quite accurate and incurs a maximum error of 6\% on both platforms for different message sizes. 
Figure~\ref{fig:simulation} also shows the breakdown of overall latency into constant and variable parts. As expected, for larger message sizes the variable component is larger (due to higher data transmission times) while smaller messages are dominated by the constant parameters.
The aim of developing this model was to understand the key sources of overhead for memory-level SM.

\begin{figure}[!t]
  \centering
\includegraphics[angle=0,width=0.95\columnwidth]{figures/6-breakdown.pdf}
  \caption{Breakdown of RDMA-based SM latency.}
\label{fig:latency_breakdown}
\end{figure}

\textbf{PCIe interface is the major performance bottleneck for memory-level SM:} Figure~\ref{fig:latency_breakdown} shows the fraction of the overall end to end latency that arises due to the PCIe interface and the RDMA network, further broken down into constant and variable components. The PCIe interface is a major source of latency and can attribute to up to 68\% of the overall latency. It is especially problematic for smaller message sizes.
Moreover, our measurements with WHISPER applications shows that small message sizes (nearly 75\% of the messages are only one cacheline long) meaning that the PCIe is a major source of performance bottleneck in memory-level SM.
This observation leads us to the conclusion that a novel interface between the processor and the RNIC with tighter integration will significantly reduce the performance overheads of memory-level SM. Next, we present a brief sketch of such a design.



%\subsection{Key sources of overhead}
%\paragraph{PCIe Transmission Overhead}


%from Scale-out NUMA: PCIe/DMA latencies limit performance. I/O bypass architectures have successfully removed most sources of latency except the PCIe bus. Studies have shown that it takes 400-500ns to communicate short bursts over the PCIe bus [21], making such transfers 7-8x more expensive, in terms of latency, than local DRAM accesses. Furthermore, PCIe does not allow for the cache-coherent sharing of control structures between the system and the I/O device, leading to the need of replicating system state such as page tables into the device and system memory. In the latter case, the device memory serves as a cache, resulting in additional DMA transactions to access the state. SoC integration alone does not eliminate these overheads, since IP blocks often use DMA internally to communicate with the main processor [5].

%Similarly, augmenting rack-scale systems with PCIe-attached RDMA controllers [21] can bring latency down to the microseconds range. However, remote access latency is still over 10x of local memory, limited by the PCIe bus and the delay of a complex RDMA-compliant ASIC. The PCIe bus also limits the bandwidth to 40Gbps (5GBps) in most configurations, which is grossly mismatched with local DRAM bandwidth that is approaching 20GBps per DDR channel.

%\paragraph{Protocol Processing Overhead}

%\paragraph{Address Translation Overhead}



